RAVEN: Radar Adaptive Vision Encoders for Efficient Chirp-wise Object Detection and Segmentation

This paper presents RAVEN, a computationally efficient deep learning architecture for FMCW radar perception. The method processes raw ADC data in a chirp-wise streaming manner, preserves MIMO structure through independent receiver state-space encoders, and uses a learnable cross-antenna mixing module to recover compact virtual-array features. It also introduces an early-exit mechanism so the model can make decisions using only a subset of chirps when the latent state has stabilized. Across automotive radar benchmarks, the approach reports strong object detection and BEV free-space segmentation performance while substantially reducing computation and end-to-end latency compared with conventional frame-based radar pipelines.

==> tables/ablation.tex <==

\begin{table*}[t]
\centering
\footnotesize
\resizebox{\textwidth}{!}{%
  \begin{threeparttable}
  \caption{Ablation study on \textbf{RADIal} segmentation task.}
  \label{tab:ablation}
  \begin{tabular}{lccccccccccccc}
    \toprule
    \textbf{Model} & \textbf{C-SSM} & \textbf{S-SSM} & \textbf{Proj} & \textbf{D-dim} & \textbf{Aggr} & \textbf{Expn} & \textbf{mIoU} & \textbf{Dice} & \textbf{mAP} & \textbf{mAR} & \textbf{Acc} & \textbf{Comp.} & \textbf{Param} \\
     &  &  &  &  &  & & \textbf{\%} & \textbf{\%} & \textbf{\%} & \textbf{\%} & \textbf{\%} & \textbf{GMACs} & \textbf{(M)} \\
    \midrule
    SSM based chirp model  & \checkmark & --         & \checkmark & 16 & -- & --   & 65.59 & 77.82 & 81.67 & 77.99 & 95.22 & 15.5 & 45.85   \\
    SSMRadNet-Proj           & \checkmark & \checkmark & \checkmark & 16 & Last    & -- & 67.99 & 79.88 & 82.37 & 79.99 & 95.57 & 0.73  & 13.40    \\
    SSMRadNet-NoProj-16      & \checkmark & \checkmark & --         & 16 & Last    & -- & 68.27 & 80.25 & 82.44 & 80.49 & 95.70 & 0.94  & 0.119  \\
    SSMRadNet-NoProj-32      & \checkmark & \checkmark & --         & 32 & Last    & -- & 70.59 & 81.85 & 83.62 & 82.23 & 96.07 & 1.21  & 0.126   \\
    SSMRadNet-FeatConv       & \checkmark & \checkmark & --         & 32 & Conv1D  & -- & 74.44 & 84.58 & 85.84 & 85.00 & 96,61 & 1.22 & 0.126   \\
    SSMRadNet-FeatPool         & \checkmark & \checkmark & --         & 32 & AvgPool & -- & 74.75 & 84.86 & 87.15 & 84.26 & 96.72 & 1.20  & 0.123  \\
    \textbf{SSMRadNet (ours) }        & \checkmark & \checkmark & --         & 32 & AvgPool & \checkmark & 78.60 & 86.77 & 88.02 & 86.81 & 97.10 & 1.52  & 0.226  \\
    \bottomrule
  \end{tabular}
  \begin{tablenotes}
    \footnotesize
    \item \textbf{C-SSM} - Chirpwise SSM, \textbf{S-SSM} - Samplewise SSM; \textbf{Proj} - Input projection; \textbf{D-dim} - Internal vector size of Mamba-SSM D-state \textbf{Aggr} - Feature aggregation strategy of samplewise-ssm. \textbf{\textit{Last}} - takes last state output, \textbf{\textit{Conv1D}} - 1D conv over samplewise features, \textbf{\textit{AvgPool}} - adaptive averagepooling  \textbf{\textit{Expn.}} - S-SSM output channels linearly expanded to 2$N_{R_X}$ before C-SSM% over samplewise \ features.
  \end{tablenotes}
  \end{threeparttable}
}
% \vspace{-5em}
\end{table*}


==> tables/detection_results.tex <==
% \begin{table}[t]
% \centering
% \footnotesize
% \resizebox{\columnwidth}{!}{%
% \begin{threeparttable}
% \caption{Overall detection performance on \textbf{RADIal}.}
% \label{tab:det_results}
% \begin{tabular}{lccccc}
% \toprule
% \textbf{Model} & \textbf{F1} & \textbf{mAP} & \textbf{mAR} & \textbf{RE (m)} & \textbf{AE ($^{\circ}$)}  \\
% \midrule
% ADCNet                    & 0.92 & 0.95 & 0.89 & 0.13 & 0.11  \\
% ADCNet (NPT)              & 0.91 & 0.96 & 0.87 & 0.12 & 0.10  \\
% ADC\,UNet                 & 0.85 & 0.88 & 0.82 & 0.18 & 0.11  \\
% ADC\,UNet (NPT)           & 0.80 & 0.83 & 0.77 & 0.19 & 0.10  \\
% Conv3D + FFT-RadNet       & 0.47 & 0.58 & 0.39 & 0.19 & 0.33  \\
% Conv3D + FFT-RadNet (NPT) & 0.37 & 0.58 & 0.27 & 0.16 & 0.46  \\
% FFT-RadNet (RD)           & ---  & 0.97 & 82.2 & 0.11 & 0.17  \\
% Pixor (PC)                & ---  & 0.96 & 0.32 & 0.17 & 0.25   \\
% Pixor (RA)                & ---  & 0.96 & 0.82 & 0.10 & 0.20   \\
% FFT-RadUNet               & 0.80 & 0.84 & 0.78 & 0.16 & 0.09  \\
% FourierNet-FFT-RadUNet    & 0.88 & 0.86 & 0.89 & 0.16 & 0.11  \\
% FourierNet-FFT-RadNet     & 0.92 & 0.91 & 0.93 & 0.14 & 0.12  \\
% SSMRadNet (Ours)       & 0.72  & 0.73  & 0.71  & 0.14   & 0.15    \\
% \bottomrule
% \end{tabular}
% \begin{tablenotes}
%   \footnotesize
%   \item RE = range error; AE = azimuth error.
% \end{tablenotes}
% \end{threeparttable}
% }
% \end{table}

==> tables/modalities.tex <==
\begin{table*}[t]
\scriptsize
\centering
\caption{Comparison of radar object detection architectures. Trade-offs:
\textcolor{green}{\checkmark} desirable, \textcolor{orange}{\textbullet} moderate, \textcolor{red}{\ding{55}} undesirable.
“Sub-frame” indicates whether the model can emit detections at sub-frame granularity (e.g., per chirp / partial frame) or run in streaming mode. {\normalfont\textsuperscript{\dag}}Attention scaling note.}
\label{tab:radar_architectures}
\setlength{\tabcolsep}{2.6pt}
\renewcommand{\arraystretch}{1.07}

\begin{tabularx}{\textwidth}{
  @{}
  >{\raggedright\arraybackslash}p{1.15cm}       % Class
  >{\raggedright\arraybackslash}p{2.40cm}       % Model
  >{\raggedright\arraybackslash}p{1.55cm}       % Input
  >{\raggedright\arraybackslash}p{1.35cm}       % Feature
  >{\raggedright\arraybackslash}X               % Core (flex)
  >{\centering\arraybackslash}p{1.05cm}         % Sub-frame
  >{\centering\arraybackslash}p{1.05cm}         % Spatial Res
  >{\centering\arraybackslash}p{0.95cm}         % Params
  >{\centering\arraybackslash}p{0.95cm}         % GMACs
  >{\centering\arraybackslash}p{1.00cm}         % Peak Mem
  >{\centering\arraybackslash}p{1.00cm}         % Latency
  @{}
}
\toprule
\textbf{Class} & \textbf{Model} & \textbf{Input} & \textbf{Feat.} & \textbf{Core} &
\makecell{\textbf{Sub-frame}\\\textbf{Inference}} &
\makecell{\textbf{Spatial}\\\textbf{Res.}} &
\textbf{Params} & \textbf{GMACs} & \textbf{Peak Mem} & \textbf{Latency} \\
\midrule

\multirow{3}{*}{Conv} &
Point-cloud Conv Detectors \cite{yang2018pixor} &
PC (CFAR) & Sparse 3D &
CNN/FPN (voxel/BEV) &
\textcolor{red}{\ding{55}} &
High \textcolor{green}{\checkmark} &
High \textcolor{red}{\ding{55}} &
High \textcolor{red}{\ding{55}} &
High \textcolor{red}{\ding{55}} &
High \textcolor{red}{\ding{55}} \\
& FFT-RadNet \cite{rebut2022radial} &
RD & 2D &
CNN encoder + FPN (angle) &
\textcolor{red}{\ding{55}} &
Mid–High \textcolor{orange}{\textbullet} &
High \textcolor{red}{\ding{55}} &
High \textcolor{red}{\ding{55}} &
High \textcolor{red}{\ding{55}} &
High \textcolor{red}{\ding{55}} \\
& ADCNet (Conv) \cite{zhang2023adcnet} &
ADC $\rightarrow$ RD & 2D &
Learnable signal proc + Conv blocks &
Limited \textcolor{orange}{\textbullet} &
High \textcolor{green}{\checkmark} &
High \textcolor{red}{\ding{55}} &
High \textcolor{red}{\ding{55}} &
High \textcolor{red}{\ding{55}} &
High \textcolor{red}{\ding{55}} \\
\midrule

\multirow{2}{*}{Attn} &
T-FFT-RadNet (Swin) \cite{giroux2023tfftradnet,liu2021swin} &
RD/RAD/ADC & 2D/3D &
Hierarchical Swin self-attn\textsuperscript{\dag} &
\textcolor{red}{\ding{55}} &
High \textcolor{green}{\checkmark} &
High \textcolor{red}{\ding{55}} &
High \textcolor{red}{\ding{55}} &
High \textcolor{red}{\ding{55}} &
High \textcolor{red}{\ding{55}} \\
& RadarFormer \cite{Dalbah2023RadarFormer} &
RA/RD (merged) & 2D &
Chirp–time merging transformer\textsuperscript{\dag} &
\textcolor{red}{\ding{55}} &
High \textcolor{green}{\checkmark} &
High \textcolor{red}{\ding{55}} &
High \textcolor{red}{\ding{55}} &
High \textcolor{red}{\ding{55}} &
High \textcolor{red}{\ding{55}} \\
\midrule

RNN &
ChirpNet \cite{sharma2024chirpnet} &
ADC (chirp/$R_x$) & 2D &
GRU sequence + small MLP &
Limited \textcolor{orange}{\textbullet} &
Mid \textcolor{orange}{\textbullet} &
Mid \textcolor{orange}{\textbullet} &
Mid \textcolor{orange}{\textbullet}} &
Mid \textcolor{orange}{\textbullet} \\
\midrule

SSM &
SSMRadNet &
ADC (sample/chirp) & 1D &
Sample- \& chirp-wise SSMs (streaming) &
Streaming \textcolor{green}{\checkmark} &
Mid \textcolor{orange}{\textbullet} &
Low \textcolor{green}{\checkmark} &
Low \textcolor{green}{\checkmark} &
Mid \textcolor{orange}{\textbullet} &
Low \textcolor{green}{\checkmark} \\
\midrule

Hybrid &
RAVEN &
ADC/Ch./chirp & 1D &
Channel-wise SSMs + antenna-attn mixer (streaming) &
Streaming \textcolor{green}{\checkmark} &
Mid–High \textcolor{green}{\checkmark} &
Low \textcolor{green}{\checkmark} &
Low \textcolor{green}{\checkmark} &
Low \textcolor{green}{\checkmark} &
Low \textcolor{green}{\checkmark} \\
\bottomrule
\end{tabularx}

\vspace{3pt}
\raggedright\scriptsize
\emph{Notes:} Qualitative levels are relative within this table. “Sub-frame” refers to output granularity finer than a full RD/RAD frame (e.g., per chirp or partial frame), or true streaming for SSMs. “Spatial Res.” is the effective spatial fidelity of features used for detection heads. 
\textsuperscript{\dag}\,Attention models scale $\mathcal{O}(N^2)$ in tokens ($N$ = slow-time/space extent).%
\end{table*}


==> tables/model_stats.tex <==
% \begin{table}[htb]
% \centering
% \footnotesize
% \resizebox{\columnwidth}{!}{%
% \begin{threeparttable}
%   \caption{Per frame runtime characteristics of radar detection models.}
%   \label{tab:model_complexity}
%   \begin{tabular}{lcccc}
%     \toprule
%     \textbf{Model}                   & \textbf{Compute} & \textbf{Params} & \textbf{Latency} & \textbf{Memory} \\
%                                      & \textbf{(GMACs)} & \textbf{(M)}    & \textbf{(ms)}    & \textbf{(GB)}   \\
%     \midrule
%     FFT-RadNet                      & 146.8  & 4.25   & 53.61  &  12.33  \\
%     FFT-RadUNet                     & 134.4  & 18.48  & ---  &  --- \\
%     ADCNet                          & ---    & 2.50   & 18.13* &  14.89  \\
%     ADC\,UNet                       & ---    & 17.30  & 8.18*  &  7.45   \\
%     FourierNet-FFT-RadUNet          & 134.4  & 19.13  &        &         \\
%     FourierNet-FFT-RadNet           & 146.6  & 4.45   &        &         \\
%     T-FFT-RadNet                    & 194    & 9.64   & 60.10  &         \\
%     ChirpNet                        & 19.7   & 57.7   & 24.06  &         \\
%     Self-Attention + ChirpNet       & 10.5   & 21.3   & 6.35   &         \\
%     Chirp-SSM                       & 15.1   & 41.6   & 63.82  &         \\
%     SSMRadNet (Ours)             & 1.2    & 0.12   & 11.86  &  0.62  \\
%     \bottomrule
%   \end{tabular}
%   \begin{tablenotes}
%     \footnotesize
%     \item Runtime characterization on an NVIDIA RTX 4060 mobile GPU.
%     % \item \textbf{*} ADCNet latency reported from \cite{zhang2023adcnet}.
%   \end{tablenotes}
% \end{threeparttable}
% }
% \end{table}


% \begin{table}[t]   % <-- change table* to table
%   \centering
%   \footnotesize
%   \caption{Runtime characteristics of radar detection models. *4060}
%   \label{tab:runtime}
%   \begin{tabular}{lccc}
%     \toprule
%     \textbf{Model}                     & \textbf{Latency} & \textbf{Throughput} & \textbf{Memory} \\
%                          & \textbf{(ms)} & \textbf{(fps)} & \textbf{(GB)} \\
%     \midrule
%         ChirpNet                       &  24.06*                   &  ---                      &  ---                 \\
%             Self Attention + ChirpNet                       &  6.35*                   &  ---                      &  ---                 \\
%     FFT-RadNet        & 53.61*                  &  18                       & 12.33                \\ % \cite{fft_radnet}
%     T-FFT-RadNet     & 60.00                  &  15                      & ---                  \\ %\cite{tfft_radnet}
%     ADCNet                             & 18.13                  &  58                       & 14.89                \\
%     ADC\,UNet                          &  8.18                  & 137                       &  7.45                \\
%     ChirpNet-SSM                       &  63.82*                   &  ---                      &  ---                 \\
%     SSMRadNet (Ours)                &  11.86*                   &   40.7                     &  0.621                 \\
%     \bottomrule

%   \end{tabular}

% \end{table}

==> tables/results.tex <==
\begin{table*}[t]
\centering
\footnotesize
\resizebox{\textwidth}{!}{%
\begin{threeparttable}
\caption{Overall segmentation and detection performance on \textbf{RADIal\cite{rebut2022radial}}.}
\label{tab:results}
\begin{tabular}{l l c c c c c c c c c c}
\toprule
\textbf{Class} 
  & \textbf{Model} 
  & \multicolumn{1}{c}{\textbf{Segmentation}} 
  & \multicolumn{5}{c}{\textbf{Detection}} 
  & \multicolumn{4}{c}{\textbf{Computational Metrics*}}\\
\cmidrule(lr){3-3} \cmidrule(lr){4-8} \cmidrule(lr){9-12} 
 &  & \textbf{mIoU} 
  & \textbf{F1} 
  & \textbf{mAP} 
  & \textbf{mAR} 
  & \textbf{RE (m)} 
  & \textbf{AE ($^{\circ}$)} 
  & \textbf{GMACs} & \textbf{Params (M)} & \textbf{Latency (ms)} & \textbf{Mem. (GB)}\\
\midrule
\multirow{11}{*}{Convolution} 
  & Pixor (PC) \cite{yang2018pixor}                & ---  & ---  & 0.96 & 0.32 & 0.17  & 0.25  & ---   & ---   & ---    & --- \\
  & Pixor (RA) \cite{yang2018pixor}                & ---  & ---  & 0.96 & 0.82 & 0.10  & 0.20  & ---   & ---   & ---    & --- \\
  & PolarNet \cite{nowruzi2020deep}                & 0.61 & ---  & ---  & ---  & ---   & ---    & ---   & ---   & ---    & --- \\
  & Conv3D + FFT-RadNet \cite{wu2024sparseradnet}  & 0.75 & 0.47 & 0.58 & 0.39 & 0.19  & 0.33   & ---   & ---   & ---    & --- \\
  & FFT-RadNet \cite{rebut2022radial}              & 0.74 & ---  & 0.97 & 0.82 & 0.11  & 0.17   & 146.8 & 4.25  & 53.61  & 12.33 \\
  & FFT-RadUNet\tnote{a}                           & 0.75 & 0.80 & 0.83 & 0.77 & 0.16  & 0.09   & 134.4 & 18.48 & ---    & --- \\
  & ADCNet \cite{zhang2023adcnet}                  & 0.79 & 0.89 & 0.93 & 0.86 & 0.13  & 0.11   & ---   & 2.50  & 18.13  & 14.89 \\
  & ADC\,UNet \cite{zhang2023adcnet}               & 0.77 & 0.85 & 0.88 & 0.82 & 0.18  & 0.11   & ---   & 17.50 & 8.18   & 7.45 \\
  & ADC\,UNet (NPT) \cite{zhang2023adcnet}         & 0.73 & 0.80 & 0.83 & 0.77 & 0.19  & 0.10   & ---   & ---   & ---    & --- \\
  & FourierNet-FFT-RadUNet\tnote{b}                & 0.78 & 0.86 & 0.84 & 0.87 & 0.16  & 0.11   & 134.4 & 19.13 & ---    & --- \\
  & FourierNet-FFT-RadNet\tnote{c}                 & 0.79 & 0.88 & 0.87 & 0.89 & 0.14  & 0.12   & 146.6 & 4.45  & ---    & ---- \\
\midrule
\multirow{2}{*}{Attention} 
  & Self Attention-based chirp model\tnote{d}      & 0.65 & ---  & ---  & ---  & ---   & ---    & 10.5  & 21.3  & 6.35   & --- \\
  & TFFT-RADNet \cite{giroux2023tfftradnet}        & 0.79 & 0.87 & 0.88 & 0.87 & 0.16  & 0.13   & 194   & 9.64  & 60.10  & --- \\
\midrule
\multirow{1}{*}{Recurrent} 
  & ChirpNet (GRU) \cite{sharma2024chirpnet}       & 0.64 & ---  & ---  & ---  & ---   & ---    & 19.7  & 57.7  & 24.06  & --- \\
\midrule
\multirow{2}{*}{SSM} 
  & SSM-based chirp model\tnote{e}                 & 0.66 & ---  & ---  & ---  & ---   & ---    & 15.1  & 41.6  & 63.82  & --- \\
  & \textbf{\textcolor{blue}{SSMRadNet (Ours)}}    & \textbf{0.79} & 0.77 & 0.83 & 0.71 & 0.14  & 0.15   & \textbf{1.6} & \textbf{0.23} & 11.86 & \textbf{0.62} \\
\bottomrule
\end{tabular}
\begin{tablenotes}
  \footnotesize
  \item RE = range error; AE = azimuth error; RA = range azimuth; PC = pointcloud.
  \item [a, b, c, d, e] [a] FFT-RadNet\cite{rebut2022radial} + UNet\cite{ronneberger2015unet}; FourierNet\cite{zhao2023cubelearn} FFT fed to [b] FFT-RadUNet, [c] FFT-RadNet; ChirpNet\cite{sharma2024chirpnet} with [d] transformer \cite{vaswani2017attention}, [e] SSM \cite{chen2024mamba} replacing GRU.
  \item *Runtime characterization on an NVIDIA RTX 4060 mobile GPU.
\end{tablenotes}
\end{threeparttable}
}
\end{table*}


==> tables/results_updated.tex <==
\begin{table*}[t]
\centering
\footnotesize
\resizebox{\textwidth}{!}{%
\begin{threeparttable}
\caption{Overall segmentation and detection performance on \textbf{RADIal\cite{rebut2022radial}}.}
\label{tab:results}
\begin{tabular}{l l c c c c c c c c c }
\toprule
\textbf{Class} 
  & \textbf{Model} 
  & \multicolumn{1}{c}{\textbf{Segmentation}} 
  & \multicolumn{5}{c}{\textbf{Detection}} 
  & \multicolumn{3}{c}{\textbf{Computational Metrics*}}\\
\cmidrule(lr){3-3} \cmidrule(lr){4-8} \cmidrule(lr){9-11} 
 &  & \textbf{mIoU} 
  & \textbf{F1} 
  & \textbf{mAP} 
  & \textbf{mAR} 
  & \textbf{RE (m)} 
  & \textbf{AE ($^{\circ}$)} 
  & \textbf{GMACs} & \textbf{Params (M)} & \textbf{Latency (ms)}\\
\midrule
\multirow{11}{*}{Convolution} 
  & Pixor (PC) \cite{yang2018pixor}                & ---  & ---  & 0.96 & 0.32 & 0.17  & 0.25  & ---   & ---   & ---     \\
  & Pixor (RA) \cite{yang2018pixor}                & ---  & ---  & 0.96 & 0.82 & 0.10  & 0.20  & ---   & ---   & ---     \\
  & PolarNet \cite{nowruzi2020deep}                & 0.61 & ---  & ---  & ---  & ---   & ---    & ---   & ---   & ---     \\
  & Conv3D + FFT-RadNet \cite{wu2024sparseradnet}  & 0.75 & 0.47 & 0.58 & 0.39 & 0.19  & 0.33   & ---   & ---   & ---     \\
  & FFT-RadNet \cite{rebut2022radial}              & 0.74 & ---  & 0.97 & 0.82 & 0.11  & 0.17   & 128.65 & 3.79  & 53.59   \\
  & FFT-RadUNet\tnote{a}                           & 0.75 & 0.80 & 0.83 & 0.77 & 0.16  & 0.09   & 116.47 & 17.85 & 38.20     \\
  & ADCNet \cite{zhang2023adcnet}                  & 0.79 & 0.89 & 0.93 & 0.86 & 0.13  & 0.11   & ---   & 2.50  & 18.13**  \\
  & ADC\,UNet \cite{zhang2023adcnet}               & 0.77 & 0.85 & 0.88 & 0.82 & 0.18  & 0.11   & ---   & 17.50 & 8.18**   \\
  & ADC\,UNet (NPT) \cite{zhang2023adcnet}         & 0.73 & 0.80 & 0.83 & 0.77 & 0.19  & 0.10   & ---   & ---   & ---     \\
  & FourierNet-FFT-RadUNet\tnote{b}                & 0.78 & 0.86 & 0.84 & 0.87 & 0.16  & 0.11   & 116.47 & 18.51 & 42.13     \\
  & FourierNet-FFT-RadNet\tnote{c}                 & 0.79 & 0.88 & 0.87 & 0.89 & 0.14  & 0.12   & 128.65 & 3.82  & 50.71     \\
\midrule
\multirow{2}{*}{Attention} 
  & Self Attention-based chirp model\tnote{d}      & 0.65 & ---  & ---  & ---  & ---   & ---    & 33.00  & 50.95  & 20.37    \\
  & TFFT-RADNet \cite{giroux2023tfftradnet}        & 0.79 & 0.87 & 0.88 & 0.87 & 0.16  & 0.13   & 81.45   & 9.67  & 46.19   \\
\midrule
\multirow{1}{*}{Recurrent} 
  & ChirpNet (GRU) \cite{sharma2024chirpnet}       & 0.64 & ---  & ---  & ---  & ---   & ---    & 24.70  & 57.72  & 27.33   \\
\midrule
\multirow{2}{*}{SSM} 
  & SSM-based chirp model\tnote{e}                 & 0.66 & ---  & ---  & ---  & ---   & ---    & 15.50  & 45.85  & 8.32   \\
  & \textbf{\textcolor{blue}{SSMRadNet (Ours)}}    & \textbf{0.79} & 0.77 & 0.83 & 0.71 & 0.14  & 0.15   & \textbf{1.52} & \textbf{0.23} & 11.86 \\
\bottomrule
\end{tabular}
\begin{tablenotes}
  \footnotesize
  \item RE = range error; AE = azimuth error; RA = range azimuth; PC = pointcloud.
  \item [a, b, c, d, e] [a] FFT-RadNet\cite{rebut2022radial} + UNet\cite{ronneberger2015unet}; FourierNet\cite{zhao2023cubelearn} FFT fed to [b] FFT-RadUNet, [c] FFT-RadNet; ChirpNet\cite{sharma2024chirpnet} with [d] transformer \cite{vaswani2017attention}, [e] SSM \cite{chen2024mamba} replacing GRU.
  \item *Runtime characterization for \textbf{ segmentation only} on an NVIDIA RTX 4060 mobile GPU. **Reported by \cite{zhang2023adcnet} on an NVIDIA RTX 3090 GPU.
\end{tablenotes}
\end{threeparttable}
}
\end{table*}


==> tables/segmentation_results.tex <==
% \begin{table}[t]
% \centering
% \footnotesize
% \begin{threeparttable}
% \caption{Overall driving space segmentation performance on \textbf{RADIal}.}
% \label{tab:seg_results}
% \begin{tabular}{lcc}
% \toprule
% \textbf{Model} & \textbf{Radar Input}  & \textbf{mIoU} \\
% \midrule
% PolarNet                  & RA   & 0.61 \\
% ChirpNet              & ADC  & 0.64 \\
% Self-Attention + ChirpNet             & ADC  & 0.65 \\
% ADCNet                    & ADC & 0.79 \\
% ADCNet (NPT)              & ADC & 0.75 \\
% ADC\,UNet                 & ADC & 0.77 \\
% ADC\,UNet (NPT)           & ADC & 0.73 \\
% Conv3D + FFT-RadNet       & RD & 0.75 \\
% Conv3D + FFT-RadNet (NPT) & RD & 0.75 \\
% FFT-RadNet (RD)           & RD  & 0.74 \\
% FFT-RadUNet\tnote{a}      & RD & 0.75 \\
% FourierNet-FFT-RadUNet\tnote{b} & ADC & 0.78 \\
% FourierNet-FFT-RadNet\tnote{c}  & ADC & 0.79 \\
% ChirpNet-SSM\tnote{d}     & ADC  & 0.66 \\
% SSMRadNet (Ours)       & ADC  & 0.75 \\
% \bottomrule
% \end{tabular}
% \begin{tablenotes}
%   \footnotesize
%   \item RD = range doppler; RA = range azimuth; PC = pointcloud.
%   \item[a] FFT-RadUNet: FFT-RadNet with UNet backbone. 
%   \item[b] FourierNet-FFT-RadUNet: FourierNet generated FFT cube passed to FFT-RadUNet
%   \item[c] FourierNet-FFT-RadNet: FourierNet generated FFT cube passed to FFT-RadNet
%   \item[d] Chirp-SSM: Chirpwise processing with SSM instead of transformer for chirp sequence modeling.
%   \item Numbers reported from the original papers: T-FFT-RadNet\cite{tfft_radnet}, ADCNet\cite{zhang2023adcnet}, ChirpNet\cite{sharma2024chirpnet}, SparseRadNet\cite{wu2024sparseradnet}.
% \end{tablenotes}
% \end{threeparttable}
% \end{table}
